Speeding up Monte Carlo Integration: Control Neighbors for Optimal Convergence

A novel linear integration rule called $\textit{control neighbors}$ is proposed in which nearest neighbor estimates act as control variates to speed up the convergence rate of the Monte Carlo procedure on metric spaces. The main result is the $\mathcal{O}(n^{-1/2} n^{-s/d})$ convergence rate -- where $n$ stands for the number of evaluations of the integrand and $d$ for the dimension of the domain -- of this estimate for H\"older functions with regularity $s \in (0,1]$, a rate which, in some sense, is optimal. Several numerical experiments validate the complexity bound and highlight the good performance of the proposed estimator.

==> preambule.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\RequirePackage{amsmath,amsfonts,amssymb,amsthm}

%\usepackage{enumerate}
%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\newcommand{\description}{}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{dsfont}
\usepackage{booktabs}  
\usepackage{setspace}
\usepackage{mathtools}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here:        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem*{theorem*}{Theorem}

\theoremstyle{definition}
\newtheorem{remark}{Remark}

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\mypar}[1]{\par\smallskip\noindent\textbf{#1}}

\def\rset{\mathbb{R}}
\def\reals{\rset}
\newcommand{\Rd}{\rset^d}
\def\cset{\mathbb{C}}
\def\zset{\mathbb{Z}}
\def\nset{\mathbb{N}}
\def\mcf{\mathcal{F}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\Prob}{\mathcal{P}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\argmax}{\operatornamewithlimits{\arg\max}}
\newcommand{\argmin}{\operatornamewithlimits{\arg\min}}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}


\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\spann}{Span}
\DeclareMathOperator{\prob}{\mathbb{P}}
\DeclareMathOperator{\expec}{\mathbb{E}}
\newcommand{\Exp}{\expec}     %expected value
\newcommand{\E}{\expec} 
\newcommand{\diff}{\mathrm{d}}
\newcommand{\1}{\operatorname{\mathds{1}}}
\newcommand{\ind}{\1} 
\newcommand{\naturals}{\mathbb{N}}

\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\ninf}[1]{\norm{#1}_\infty}
\newcommand{\abs}[1]{\left|{#1}\right|}

\newcommand{\oh}{\operatorname{o}}
%\newcommand{\Oh}{\operatorname{O}}
\newcommand{\Oh}{\mathcal{O}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MACROS FOR INTEGRANDS/MEASURES/DENSITIES %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\func}{\varphi}
\newcommand{\meas}{\mu}
\newcommand{\dens}{f}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\Leb}{\operatorname{\lambda}} % Lebesgue measure
\newcommand{\vol}{\operatorname{\nu}} 

\newcommand{\mani}{\mathcal{M}_g}
\newcommand{\inj}{\operatorname{inj}}
\newcommand{\rad}{\operatorname{rad}}
\newcommand{\ms}{M}
\newcommand{\cbr}[1]{\left\{ #1 \right\}}
\newcommand{\rbr}[1]{\left( #1 \right)}
\newcommand{\sbr}[1]{\left[ #1 \right]}
\newcommand{\propdifflooNN}{3}
\newcounter{assumpnum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\hgni}{\hat{\func}_{n}^{(i)}}
\newcommand{\Nni}{\hat{N}_{n}^{(i)}}
\newcommand{\Nn}{\hat{N}_{n}}
\newcommand{\munNN}{\hat{\meas}_{n}^{\mathrm{(NN)}}}
\newcommand{\munNNloo}{\hat{\meas}_{n}^{\mathrm{(NN-loo)}}}
\newcommand{\htgni}{\hat{\tilde{\func}}_{n}^{(i)}}


\newcommand{\tX}{\tilde{X}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\xcross}{\textcolor{red}{$\times$}}
\newcommand{\greenV}{\textcolor{britishracinggreen}{$\checkmark$}}

\newcommand{\Pn}{\frac{1}{n} \sum_{i=1}^n}

\definecolor{auburn}{rgb}{0.43, 0.21, 0.1}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{burntumber}{rgb}{0.54, 0.2, 0.14}
\definecolor{carmine}{rgb}{0.59, 0.0, 0.09}
\definecolor{aurometalsaurus}{rgb}{0.43, 0.5, 0.5}
\definecolor{gray}{rgb}{0.4, 0.4, 0.4 }
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
\definecolor{darkteal}{rgb}{0, 0.35, 0.35}
\newcommand{\js}[1]{\textcolor{darkteal}{\upshape\small\sffamily [{#1}]}}
\newcommand{\rl}[1]{\textcolor{britishracinggreen}{\upshape\small\sffamily [RL -- {#1}]}}
\newcommand{\fp}[1]{\textcolor{carmine}{\upshape\small\sffamily [FP -- {#1}]}}
\newcommand{\mdf}[1]{\bgroup\color{cerulean}{#1}\egroup}
\newcommand{\mdff}[1]{\bgroup\color{carmine}{#1}\egroup}
